Challenges in Procedural Multimodal Machine Comprehension:A Novel Way To Benchmark

We focus on Multimodal Machine Reading Comprehension (M3C) where a model is expected to answer questions based on given passage (or context), and the context and the questions can be in different modalities. Previous works such as RecipeQA have proposed datasets and cloze-style tasks for evaluation. However, we identify three critical biases stemming from the question-answer generation process and memorization capabilities of large deep models. These biases makes it easier for a model to overfit by relying on spurious correlations or naive data patterns. We propose a systematic framework to address these biases through three Control-Knobs that enable us to generate a test bed of datasets of progressive difficulty levels. We believe that our benchmark (referred to as Meta-RecipeQA) will provide, for the first time, a fine grained estimate of a model's generalization capabilities. We also propose a general M3C model that is used to realize several prior SOTA models and motivate a novel hierarchical transformer based reasoning network (HTRN). We perform a detailed evaluation of these models with different language and visual features on our benchmark. We observe a consistent improvement with HTRN over SOTA (~18% in Visual Cloze task and ~13% in average over all the tasks). We also observe a drop in performance across all the models when testing on RecipeQA and proposed Meta-RecipeQA (e.g. 83.6% versus 67.1% for HTRN), which shows that the proposed dataset is relatively less biased. We conclude by highlighting the impact of the control knobs with some quantitative results.

==> intro.tex <==
\section{Introduction}
Multi-Modal Machine Comprehension ($M^3C$) is a recent research direction that extends the traditional Machine Reading Comprehension (MRC) by introducing multimodality in the context or the questions. Even though modality has several associations, images, text, and videos are widely used in the vision and language community. 

MRC is a form of Question Answering (QA) task that provides unstructured knowledge in context (short paragraphs). VQA is a form of MRC where the question is in natural language form, and the context is visual. Contrary to these tasks, $M^3C$  introduces multimodality in the context or the questions. One specific type of $M^3C$ deals with the procedural description of steps in the passage designed to achieve a particular goal.  Procedural $M^3C$ differs from the traditional MRC in several ways: 1) presence of multi-modal data in the context, 2) $M^3C$ is a mini-story described as a step-by-step procedure, 3) the text length and count of images vary across steps. As with the internet, we are inundated with how-to guides procedurally describing cooking recipes, wikiHow,  crafting, learning tools, woodwork, etc.  The apparent next research direction is to design models that can solve these $M^3C$ QA tasks. 
 Models aimed at solving $M^3C$ can answer arbitrary questions about any procedures, should comprehend the overall idea provided by both text and images, capture the semantic correlation between text-to-image in every step, determine the entities, infer relations among the steps, and be aware of changes in the states of these entities. The above is inherently an uphill task for the current models designed to succeed in MRC. 

% Tasks involving language-and-vision seek to design model that comprehends both image, text and also the range of semantic details in the image mentioned in the text. These models serve as a test-bed for demonstrating the understanding capabilities by evaluating them on a question-answer set about documents that contain both visual and textual ?.
% Current multimodal tasks are limited by their data structure of paired image and text such as  captioning (Chen et al., 2015), visual question answering (Antol et al., 2015), and visual reasoning (Zellers et al., 2019). Over last few years, the research community has seen an overpouring contribution towards the above mentioned tasks by adding more datasets or by providing improved solutions.


Our work here dives into the recently proposed step-wise cooking recipes dataset RecipeQA ().  We begin by asking if the dataset released and the Cloze style QA evaluation method are correct for measuring comprehension of any model.  
...
We instead propose to evaluate this task on multiple datasets that are generated from a meta dataset. Controlling the knobs of the proposed framework generate these multiple datasets to yield sets from easy to difficult to probe currentM3Csys-terms capacity to learn.• We finally show that previously proposed models are unable to take full advantage of the context provided. We show that it is easy to gain large improvements by improving upon the visual features. We also propose a hierarchical transformer-based model that can beat the previous SOTA baseline without fully utilizing the comprehension.

To sum up, our contributions are categorized into three primary folds:
\begin{itemize}

    \item 
    
    We present an in depth study in solving Multi-Modal Machine Comprehension (MMC) task. 
    
    Our finding reveal critical gaps in how this task has been evaluated while raising the question: \textit{Is Question Answering task the right way to evaluate a machine's capability to understand and solve MMC task?} 
    
    \item We instead propose to evaluate this task on multiple datasets that are generated from a meta dataset. These multiple datasets are generated by controlling the knobs of the proposed framework so as to yield sets from easy to difficult to probe current $M^3C$ systems capacity to learn.
    
    \item We finally show that previously proposed models are unable to take full advantage of the context provided. We show that it is easy to gain large improvements by improving upon the visual features. We also propose a hierarchical transformer based model that is able to beat previous SOTA baseline without fully utilizing the comprehension.
    
    % \item The query sequence plays a vital role in models learning to find the best fit answer from the choice list.
\end{itemize}
